Fifty Shades of Congestion Control: A Performance and Interactions Evaluation

Congestion control algorithms are crucial in achieving high utilization while preventing overloading the network. Over the years, many different congestion control algorithms have been developed, each trying to improve in specific situations. However, their interactions and co-existence has, to date, not been thoroughly evaluated, which is the focus of this paper. Through head-to-head comparisons of representatives from loss-based, delay-based and hybrid types of congestion control algorithms, we reveal that fairness in resources claimed is often not attained, especially when flows sharing a link have different RTTs.

==> csv/introduction.tex <==
%New technologies such as 5G will enable the deployment of applications with much stricter Quality of Service (QoS) requirements than today's applications. %As a consequence, dependency of critical services, such as healthcare and/or transport, on network performance will increase significantly. %Thus, many aspects of the modern life will become unimaginable without a well functioning Internet. 
%Industry analysts also predict that by 2020, 50 billion devices will exchange information over the Internet, with smart cars, machines, homes appliances, and others joining the asdcomputers and phones in use today \cite{ericsson2011more}. 
In the wake of the %resulting 
growing demand for higher bandwidth, higher reliability, and lower latency, novel congestion control algorithms have been developed. %might not be appropriate anymore, or at least require some re-thinking. 
%To answer specific requirements such as low-latency or high reliability, multiple congestion control algorithms have been developed over the past few years. %All of them claim to operate at a point where throughput is maximized while minimizing queuing delay and packet loss. 
For example, in 2016, Google published its bottleneck bandwidth and round-trip time (BBR) congestion control algorithm \cite{3022184}, claiming it was able to operate without %creating packet loss or 
filling buffers. %BBR does this by periodically estimating the propagation Round-Trip Time (RTT) and the available bandwidth. 
Around the same time, TCP LoLa \cite{lola} and TIMELY \cite{TIMELY} were proposed, focusing on low latency and bounding of the queuing delay. % by using RTT measurements, respectively.  
Moreover, new transport protocols such as QUIC allow the implementation of algorithms directly in user space, which facilitates quick development of new transport features. 
However, \emph{congestion control algorithms have been typically developed in isolation}, without thoroughly investigating their behaviour in the presence of other congestion control algorithms, which is the goal of this paper. 
%In addition,
%\todo{add a part that existing evaluations just compare two algorithms and are mostly simulations.}
%Our focus in this paper is on the interactions between different flavours of TCP. 

%\todo{add contributions}

% Contributions
In this paper, we first divide existing congestion control algorithms into three groups: loss-based, delay-based, and hybrid. We study their interactions based on experiments in a testbed. We observe multiple fairness issues, among flows of the same group, across groups, as well as when flows having different RTTs were sharing a bottleneck link.  We find that delay-based, as well as hybrid algorithms, suffer from a decrease in performance when competing with flows from the loss-based group, making them unusable in a typical network where the majority of flows will rely on a loss-based algorithm. Not only do they get an unfair share of the available bandwidth, but they also suffer from a huge increase in the observed delay when the loss-based algorithms fill the queues. In addition, the observe that convergence times are large (up to $60s$), and possibly larger than the duration time of a typical flow for many applications. Finally, we find that hybrid algorithms, such as BBR, not only favour the flow with a higher RTT at the expense of the other flows, but they also cannot maintain a low queuing delay as promised.

In Section %\ref{Sec_Congestion_Control} and 
\ref{Sec_Classification}, we provide an overview of congestion control mechanisms. These algorithms are classified in 3 main groups, namely loss based, delay based, and hybrid. In Section \ref{Sec_eval}, we (1) identify a set of key performance metrics to compare them, (2) describe our measurement setup, and (3) present our measurement results. %different congestion control algorithms. 
